Video Captioning with Boundary-aware Hierarchical Language Decoding and Joint Video Prediction

The explosion of video data on the internet requires effective and efficient technology to generate captions automatically for people who are not able to watch the videos. Despite the great progress of video captioning research, particularly on video feature encoding, the language decoder is still largely based on the prevailing RNN decoder such as LSTM, which tends to prefer the frequent word that aligns with the video. In this paper, we propose a boundary-aware hierarchical language decoder for video captioning, which consists of a high-level GRU based language decoder, working as a global (caption-level) language model, and a low-level GRU based language decoder, working as a local (phrase-level) language model. Most importantly, we introduce a binary gate into the low-level GRU language decoder to detect the language boundaries. Together with other advanced components including joint video prediction, shared soft attention, and boundary-aware video encoding, our integrated video captioning framework can discover hierarchical language information and distinguish the subject and the object in a sentence, which are usually confusing during the language generation. Extensive experiments on two widely-used video captioning datasets, MSR-Video-to-Text (MSR-VTT) \cite{xu2016msr} and YouTube-to-Text (MSVD) \cite{chen2011collecting} show that our method is highly competitive, compared with the state-of-the-art methods.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> approach_-_Copy.tex <==
\section{Method}

Let $\mathbf{f}=(f_0,\cdots, f_{N-1})$ be a sequence of video frames, where $f_i$ is the image at time step $i$, and $N$ is  the length of the sequence. The video captioning task is to generate a text $\hat{\mathbf{Y}}=\{\hat{Y}_0, \cdots, \hat{Y}_{T-1}\}$ that describes the video, where $\hat{Y}_t\in \mathcal{D}$ is a word predicted from a vocabulary $\mathcal{D}$, and $T$ denotes the number of words in the description. %In this paper, we consider the problem of learning to generate video description $\hat{\mathbf{Y}}=\{\hat{Y}_0, \cdots, \hat{Y}_{T-1}\}$ for a video sequence $\mathbf{f}=\{f_0,\cdots, f_{N-1}\}$, where $\hat{Y}_t\in \mathcal{D}$ is the predicted word, $\mathcal{D}$ is the dictionary, $T$ denotes the sequence length, $f_i$ is the extracted image frame from video, and $N$ denotes the frame sequence length. 

\begin{figure*}[ht]
	\centering
	\vspace{2mm}
	\includegraphics[width=0.85\linewidth]{vtt_main.png} %\linewidth
	\caption{Illustration of our proposed framework. Our model contains two training paths: one is for caption generation, and the other is for video prediction. Note that the parameter of two video encoder as well as the attention model are share across two training paths.}
	\label{fig:top}
\end{figure*}
Figure~\ref{fig:top} shows our proposed framework for video caption generation. It consists of three parts: (i) video feature extraction, (ii) language prediction, and (iii) video prediction. As shown in Figure~\ref{fig:top}(a), a pre-trained CNN is used to encode each  video frame $f_i \in \mathbf{f}$ into a feature vector $v_{f_i}$ yielding video features $\mathbf{v}_f=(v_{f_0},\cdots, v_{f_{N-1}})$. Specifically, we obtain the image features $v_{f_i}$ by performing a mean-pooling over the spatial image features in the final convolutional layer of a CNN that is pre-trained on a large image recognition dataset like ImageNet \cite{deng2009imagenet}. The extracted image features are then fed into an RNN encoder-decoder framework that generates a caption by encoding the image features sequentially. In the following, we first describe a simple encoder-decoder framework as a baseline reference for video captioning. Then we present our proposed multi-task learning approach with improved attention mechanism. 



% $\mathbf{v}_f=(v_{f_0},\cdots, v_{f_{N-1}})$, where $v_{f_i}=\text{CNN}_{\text{Enc}}(f_i)$, for $i \in [0,N-1]$.      

%For {video feature extraction} (),   encode  into  features $\mathbf{v}_f=(v_{f_0},\cdots, v_{f_{N-1}})$, where $v_{f_i}=\text{CNN}_{\text{Enc}}(f_i)$, for $i \in [0,N-1]$. 





% , and then introduce our proposed multi-task learning approach which adopts an additional video prediction procedure to improve the video encoding.

%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=\linewidth]{v2v_one_step.png}
%	\caption{The structure of the boundary-detection based video encoder.}\label{fig:bd_video}
%\end{figure}

\subsection{Baseline Video Caption Generation Model}\label{sec:baseline}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=\linewidth]{baseline.png} %\linewidth
	\caption{Our encoder-decoder baseline with a bi-directional GRU encoder.}
	\label{fig:baseline}
\end{figure}


Our baseline video captioning model (Figure \ref{fig:baseline}) is similar to the standard encoder-decoder RNN model used in machine translation \cite{sutskever2014sequence}. To model the temporal information in
a video, we employ a bi-directional RNN with GRU recurrent cells~\cite{cho2014learning} as the encoder. The operations of the encoder ($\text{GRU}_{\text{Enc-bi}}^v$) can be expressed as:

\begin{equation}
(v_{0}^{\text{bi}},\cdots, v_{N-1}^{\text{bi}}) = \text{GRU}_{\text{Enc-bi}}^v ([v_{f_0},\cdots, v_{f_{N-1}}]) \label{eq:gru_base}\\
%	h_t^l, o_t^l =&~ \text{GRU}_{\text{Dec}}^l(h_{t-1}^l, y_{t-1}^l)
\end{equation}

\noindent where $v_i^{\text{bi}}$ is the concatenated output of the bidirectional GRU video encoder at time step $i$. Like LSTMs \cite{hochreiter1997long}, GRUs are good at memorizing long sequences, but computationally more efficient.

The decoder $\text{GRU}_{\text{Dec}}^l$ is a unidirectional RNN with GRU cells, which is fed with the \emph{average} of the encoded vectors  $\{v_{0}^{\text{bi}},\cdots, v_{N-1}^{\text{bi}}\}$  as the input at the first time step ($t=0$). The decoding step at time step $t$ can be expressed as: 

\begin{equation}
%	(v_{0}^{\text{bi}},\cdots, v_{N-1}^{\text{bi}}) = \text{GRU}_{\text{Enc-bi}}^v ([v_{f_0},\cdots, v_{f_{N-1}}])\\
h_t^l, o_t^l = \text{GRU}_{\text{Dec}}^l(h_{t-1}^l, y_{t-1})\\
%Y_t&\sim \text{argmax}(\mathbf{W}_\text{o}^\text{l} o_t^{\text{gate}}+\mathbf{b}_\text{o}^\text{l})
\end{equation}
\begin{equation}
Y_t\sim \text{argmax}(\mathbf{W}_\text{o}^\text{l} o_t^{\text{l}}+\mathbf{b}_\text{o}^\text{l})
\end{equation}
where $h_t^l$ is the hidden state of $\text{GRU}_{\text{Dec}}^l$, $o_t^l$ is the output of $\text{GRU}_{\text{Dec}}^l$. $Y_t$ is the index of rhe predicted word which has the highest probability in the Softmax process, $y_{t-1}=\mathbf{W}_eY_{t-1}$ is the embedding of previous word $Y_{t-1}$, and $Y_t$ is a word index drawn from the dictionary according to the output probability of Softmax.
%\alert{Shi/Gu: define what are $h_{t-1}^l, y_{t-1}^l, h_t^l, o_t^l$ and also define the output Softmax distribution explicitly along with the loss function}


%Our baseline video captioning model, as shown in \red{Figure \ref{},}, is similar to the standard encoder-decoder RNN model used in machine translation \cite{sutskever2014sequence}. \alert{Shi: we need a figure of our baseline model}. To model the temporal information in
%a video, we employ a bi-directional RNN with GRU recurrent cells~\cite{cho2014learning} as the encoder. The operations of the encoder ($\text{GRU}_{\text{Enc-bi}}^v$) can be expressed as:

%\begin{equation}
%	(v_{0}^{\text{bi}},\cdots, v_{N-1}^{\text{bi}}) = \text{GRU}_{\text{Enc-bi}}^v ([v_{f_0},\cdots, v_{f_{N-1}}]) \label{eq:gru-rnn}
%	h_t^l, o_t^l =&~ \text{GRU}_{\text{Dec}}^l(h_{t-1}^l, y_{t-1}^l)
%\end{equation}

%\noindent where $v_i^{\text{bi}}$ is the concatenated output of the bidirectional GRU video encoder at time step $i$. \blue{Like LSTMs \cite{hochreiter1997long}, GRUs are good at memorizing long sequences, but computationally more efficient.}  

%The decoder $\text{GRU}_{\text{Dec}}^l$ is a unidirectional RNN with GRU cells, which is fed with the \emph{average} of the encoded vectors  $\{v_{0}^{\text{bi}},\cdots, v_{N-1}^{\text{bi}}\}$  as the input at the first time step ($t=0$). The decoding step at time step $t$ can be expressed as: 

%\begin{equation}
%	(v_{0}^{\text{bi}},\cdots, v_{N-1}^{\text{bi}}) = \text{GRU}_{\text{Enc-bi}}^v ([v_{f_0},\cdots, v_{f_{N-1}}])\\
%	h_t^l, o_t^l = \text{GRU}_{\text{Dec}}^l(h_{t-1}^l, y_{t-1}^l)
%\end{equation}

%\alert{Shi/Gu: define what are $h_{t-1}^l, y_{t-1}^l, h_t^l, o_t^l$ and also define the output Softmax distribution explicitly along with the loss function}




%a one-layer GRU as the decoder~\cite{bahdanau2014neural}, called $\text{GRU}_{\text{Enc-bi}}^v$ and $\text{GRU}_{\text{Dec}}^l$ respectively.


%The operations of the encoder ($\text{GRU}_{\text{Enc-bi}}^v$) and the decoder ($\text{GRU}_{\text{Dec}}^l$) can be expressed as:

%\begin{align}
%	(v_{0}^{\text{bi}},\cdots, v_{N-1}^{\text{bi}}) =&~\text{GRU}_{\text{Enc-bi}}^v ([v_{f_0},\cdots, v_{f_{N-1}}])\\
%	h_t^l, o_t^l =&~ \text{GRU}_{\text{Dec}}^l(h_{t-1}^l, y_{t-1}^l)
%\end{align}

The baseline model has two major problems. First, the language decoder generates words based on a single global video feature vector (i.e., $\bar{v}^{\text{bi}} = avg(v_{0}^{\text{bi}},\cdots, v_{N-1}^{\text{bi}})$). However, since a caption describes the whole video, some words in the caption only relate to a specific portion of the video. For example, consider the sequence of actions in Figure~\ref{fig:top}. The textual entity \emph{woman} is present (as an image object) only in the first few image frames, and the entity \emph{egg} comes only in the later part of the video. Decoding words based on a single global video representation could lead to sub-optimal results due to irrelevant information in the encoded feature vector, especially when the video sequence is long.    


%However, in most cases, some words are related only to a small portion of the video (for example, consider woman/egg in Figure~\ref{fig:top}). 

The second problem is that the simple GRU-based video encoder lacks sufficient temporal supervision to be able to correctly capture the event sequence in a video. Ideally, we would want the video encoder to learn representations that are useful for not only caption generation, but also to maintain the temporal information in videos \cite{pasunuru2017multi}. In the following, we present our approach to address these limitations of the baseline model.     


\subsection{Our Approach}

To focus on the relevant frames of a video while decoding caption words, we propose a novel hierarchical language decoder with global visual attention. Additionally, we propose to use a boundary-aware video encoder \cite{baraldi2016hierarchical} to separate out the actions (e.g., `woman handling a pan' and `adding eggs to the pan' in Figure~\ref{fig:top}) in a video. %along with a boundary-aware GRU (B-GRU) layer. 
To better capture temporal information in the encoded video features, we include an additional training path where we learn representations by generating a portion of the video sequence. In the following, we describe our proposed methods in detail. 


%\red{Meanwhile, the B-GRU we propose can also be beneficial for avoiding the misleading of language such as the confusion between "dog" and "sheep" we mentioned in the introduction, since it generates the words which has more direct relation with each other.} 

\subsubsection{Hierarchical Language Decoding with Visual Attention}

Figure~\ref{fig:top}(b) illustrates our caption generation model for a given sequence of image features $\mathbf{v}_f=(v_{f_0},\cdots, v_{f_{N-1}})$. The spatial image features are first encoded into a temporal sequence of feature representations $(v_{0}^{\text{bi}},\cdots, v_{N-1}^{\text{bi}})$ with a GRU-based RNN  following Eq.~\eqref{eq:gru_base}. The model then uses a hierarchical language decoder with a visual attention layer to selectively attend to encoded video features $\mathbf{v}^{\text{bi}} =\{v_{0}^{\text{bi}},\cdots, v_{N-1}^{\text{bi}}\}$ while generating the caption words. 

%\blue{We also propose to use a boundary-aware GRU encoder. In the interest of coherence, we first describe the attention mechanism used by the hierarchical decoder, then we present the boundary-aware video encoder} 
\begin{figure}[t]
	\centering
	\includegraphics[width=0.85\linewidth]{v2t_one_step.png}
	\caption{The structure of our proposed Binary Gated Recurrent Unit.}\label{fig:bgru}
	\vspace{-2mm}
\end{figure}
Figure~\ref{fig:bgru} shows our  proposed language decoder, specifically designed for video captioning. The decoder comprises two intertwined GRU layers. {The GRU at the top ($\text{GRU}_{\text{Dec}}^l$) works as a global (caption-level) language model, while the GRU at the bottom ($\text{B-GRU}$) works a local (phrase-level) language model. The B-GRU generates words to form consistent phrases (e.g., `A woman', `adding eggs in a pan') by attending on the relevant portion of the video, while the global GRU guides the B-GRU to generate globally consistent sentences.}  

%\blue{we characterize the first GRU ($\text{GRU}_{\text{Dec}}^l$) as well as the attention module as the top-down visual attention network, and the second improved GRU, $\text{B-GRU}$, as the language model.}

The inputs to $\text{GRU}_{\text{Dec}}^l$ consist of its previous hidden state $h_{t-1}^l$ and $\bar{h}_{t-1}^{\text{gate}}$ of the $\text{B-GRU}$: 
\begin{align}
h_t^l&= \text{GRU}_{\text{Dec}}^l(\bar{h}^{\text{gate}}_{t-1},h_{t-1}^l)\label{eq:lang0}
\end{align}

We use the hidden state $h_{t}^l$ at each time step $t$ to generate an attention (or context) vector as follows: 

\begin{equation}
{v_t^{\text{att}} = g_{\text{att}}(\mathbf{v}^{\text{bi}},h_{t}^{l})    =        \sum_{n=0}^{N-1} \alpha^t_n \cdot v^{\text{bi}}_{n} }
\label{eq:att_0}
\end{equation}
where $\alpha^t_n$ is the attention weight computed as follows:

\begin{align}
A^t_{n} &= \text{tanh}(\mathbf{W}_h^e h_{t}^{l}  + \mathbf{W}^e_v v_{n}^{\text{bi}}) \\
\mathbf{\alpha^t}&= \text{softmax}(\mathbf{W}_{a} \mathbf{A}^{t}+\mathbf{b}_{a})
\end{align}
with $\mathbf{W}_h^e$, $\mathbf{W}^e_v$, and $\mathbf{W}_{a}$ being the weight matrices, and $\mathbf{b}_{a}$ being the bias vector.  


%where the attended video feature is used as input to the B-GRU.

The input to the B-GRU consists of its previous hidden state $h^{\text{gate}}_{t-1}$, the attention vector $v_t^{\text{att}}$, the updated hidden state $h^l_{t}$, and the embedding of the previous word $y_{t-1}$:



\begin{equation}
o^{\text{gate}}_t, h^{\text{gate}}_t, \bar{h}^{\text{gate}}_t = \text{B-GRU}\left(v_t^{\text{att}}, h^l_{t}, h^{\text{gate}}_{t-1}, y_{t-1}\right)\label{eq:lang1}
%Y_t&\sim \text{argmax}(\mathbf{W}_\text{o}^\text{l} o_t^{\text{gate}}+\mathbf{b}_\text{o}^\text{l})
\end{equation}

Finally, the output layer of the decoder RNN predicts the words:
\begin{equation}
%h^{\text{gate}}_t, o^{\text{gate}}_t&= \text{B-GRU}\left(c_t, h^l_{t}, h^{\text{gate}}_{t-1}, y_{i-1}\right)\label{eq:lang1}\\
Y_t \sim \text{argmax}(\mathbf{W}_\text{o}^\text{l} o_t^{\text{gate}}+\mathbf{b}_\text{o}^\text{l})
\end{equation}
where $\mathbf{W}_\text{o}^\text{l}$ is the weight matrix and $\mathbf{b}_\text{o}^\text{l}$ is the bias vector at the output layer, and $Y_t$ is the index of the predicted word which has the highest probability. In the following, we describe our proposed binary GRU unit in detail. 

%$Y_t$ is the index of the predicted word which has the highest probability, $y_t=\mathbf{W}_eY_{t-1}$ is the embedding of previous word $Y_{t-1}$, and 

\paragraph{\textbf{Binary Gated Recurrent Unit (B-GRU)}}
Here, the proposed B-GRU can generate the words which has more direct relation with each other. 
In an original $\text{GRU}$, there are two gates: update gate $z_t$ and reset gate $r_t$.
The update gate  $z_t$ controls the contribution of hidden layer $h_{t-1}^l$ in the output.
The reset gate $r_t$ controls the forget rate of $h_{t-1}^l$ when computing the candidate activation.
In this paper, we also introduce a new gate, called binary gate, which generates a signal number $s_t \in \{ 0, 1 \}$ by comparing the local language information with the global one.
During sentence prediction, $\text{GRU}_{\text{Dec}}^l$ contains global information about the language generation by encoding each predicted phrase, and B-GRU is used to generate words in a group with local language information.
So we merge the hidden state of them to a signal vector and translate it into a real number between 0 to 1. Then we use a step function to change the signal number to \{0,1\}.

When we start a sentence generation, we initialize the hidden layer of $\text{GRU}_{\text{Dec}}^l$ with $v_{N-1}^{\text{bd}}$. Thus, the $\text{GRU}_{\text{Dec}}^l$ get the global understanding of the video.
At each time step, the $\text{GRU}_{\text{Dec}}^l$ is encoded with $\bar{h}^{\text{gate}}_{t-1}$ which contains the local language information. Thus, $h^l_t$ (the output of $\text{GRU}_{\text{Dec}}^l$) contains the both the global inforamtion of video side and language side. Thus, we use it to guide a soft attention model to generate a better attened vector with the understanding  from both sides. Then we send the attended vector to the B-GRU as a input. Only an attened vector is not enough because the model will be lack of necessary language information when we re-initialize the hidden state of B-GRU. Thus, we also input the $h^l_t$ to give the B-GRU some weak information of the language. Then we introduce the $y_{t-1}$ which is the language embedding of the previous word to B-GRU to keep the local lanugage dependency in the language decoding. In this way the hierarchical language model force the $\text{GRU}_{\text{Dec}}^l$ to generate a global fused feature to give a high-level inforamtion for soft attention model and B-GRU. And the B-GRU is forced to generate the words with more strong dependency.

Figure~\ref{fig:bgru} shows the structure of B-GRU, and its translation formulations can be shown as follows:
\begin{align}
%\bar{h}^{\text{gate}}_{t-1} &= s_t \cdot h^{\text{gate}}_{t-1}
z_t &= \sigma(\mathbf{W}_z[h_t^l;y_{t-1};v_t^{att};h^{\text{gate}}_{t-1}]+\mathbf{b}_z)\label{eq:9}\\
r_t &= \sigma(\mathbf{W}_r[h_t^l;y_{t-1};v_t^{att};h^{\text{gate}}_{t-1}]+\mathbf{b}_r)\\
\tilde{h}_t&=\tanh(\mathbf{W}[r_t \cdot h^{\text{gate}}_{t-1}; h_t^l;y_{t-1};v_t^{att}]) \\
\label{eq:13}
o^{\text{gate}}_t &=  z_t \cdot\tilde{h}_t + (1 - z_t) \cdot h^{\text{gate}}_{t-1}\\
s_t &=\tau(\sigma(\mathbf{W}_so^{\text{gate}}_{t} + \mathbf{W}_m h_t^l +\mathbf{b}_s))\\
{h}^{\text{gate}}_t &=  s_t \cdot o^{\text{gate}}_t\\
\bar{h}^{\text{gate}}_t& = (1 - s_t) \cdot o^{\text{gate}}_t
\label{eq:16}
\end{align}
where $h^{\text{gate}}_{t-1}$ is  hidden state of B-GRU of last time step, $z_t$ is update gate and $r_t$ is the rest gate, $s_t$ is the split signal generated by the binary gate.
The step function $\tau$ is the defined as follows:
\begin{align}
\tau(\sigma(x)) = \begin{cases} 1, & \mbox{if } \sigma(x) > 0.5 \\ 0, & \mbox{otherwise} \end{cases}
\label{eq:deterministic_step}
\end{align}
where $\sigma(\cdot)$ is the sigmoid function.
 

%Since the B-GRU refreshes the hidden layer to keep the 
Since the B-GRU will refresh the hidden layer when the binary gate detects the end of a phrase, an output of B-GRU $o^{\text{gate}}_{t-1}$ only contains the information from the end of the last phrase to the word the model predicts currently according to the Eq. (\ref{eq:13}).
At each time step, $\bar{h}^{\text{gate}}_{t-1}$ contained local language information is sent to $\text{GRU}_{\text{Dec}}^l$ to guide it to generate a fused visual feature relative to received local language information as an additional video information for language decoding.



When $s_t = 0$ in the B-GRU, it means that there is no strong relationship between new predicted word and previous words. In this situation, $h^{\text{gate}}_{t-1}$ will be re-initialized before inputted to $\text{B-GRU}$. When $s_t = 1$, which means the new predicted word should be in the same phrase with previous words, $h_t^{\text{gate}}$ is generated with the previous hidden state \(h_{t-1}^{\text{gate}}\). 

%In that situation, $o^{\text{gate}}_{t}$ only contains the information from the end of the last phrase to the word the model predicts currently according to the Equ. 20.
%At each time step, $o^{\text{gate}}_{t}$ will be fed back to $\text{GRU}_{\text{Dec}}^l$ to guide it to generate a fused visual feature relative to received local language information as an additional video information for language decoding.
%Since the fused feature only contains the language information predicted till now, the model can not directly use it to predict the next phrase. 
%Thus, if the attention vector $g_{\text{att}}(\mathbf{v}_f^{\text{bi}},h_{t}^l)$ and $h_t^l$ are sent into B-GRU, we can predict a representative feature with elements of the new phrase in it as the $GRU_\text{Dec}^v$ does in video prediction process. However, the feature can hardly represent a phrase directly because the feature contains mass information comparing with a phrase. Therefore, we introduce the embedding of the previous word into B-GRU to pick out an accurate phrase representation from the redundant information for B-GRU.
%\noindent\textbf{Binary Gated Recurrent Unit.}

%Since the B-GRU will re-initialize the hidden state when the binary gate detects the end of a phrase, an output of B-GRU $o^{\text{gate}}_{t-1}$ only contains the information from the end of the last phrase to the word the model predicts currently according to the Eq. (13).



\subsubsection{Boundary-aware Video Encoder.}

To separate out the actions in a video, in addition to video encoding with attention, we also consider a boundary-aware video  encoder \cite{baraldi2016hierarchical}. We denote this boundary-aware encoder with $\text{GRU}_{\text{Enc-bd}}^v$. 

%The input to boundary-aware video encoder consists of extract frame features 
%$\mathbf{v}_f$:

\begin{align}
\{v_{0}^{\text{bd}},\cdots, v_{N-1}^{\text{bd}}\}=&\text{GRU}_{\text{Enc-bd}}^v ([v_{f_0},\cdots, v_{f_{N-1}}])
\end{align}

\noindent The {transformation} functions for $\text{GRU}_{\text{Enc-bd}}^v$ are defined as follows:


\begin{align}
% v_{bd}=g_{BD}(v^{f})
h_{t}^{\text{bd}_0} =& \text{GRU}_{\text{Enc-bd}}^{v0}(v_{f_t}, h_{t-1}^{\text{bd}_0})\\
%, o_t^{\text{bd}_0}
\beta =& \tau \left( \sigma \left( f_{\text{bd}}  ({v_{f_t}},h_{t-1}^{\text{bd}_0}) \right) \right)  \\ 
h_t^{\text{bd}_0}=& h_t^{\text{bd}_0}\cdot \left(1-\beta \right)\\
h_{t}^{\text{bd}}, {v_t^{\text{bd}}} =& \text{GRU}_{\text{Enc-bd}}^{v1}(h_t^{\text{bd}_0} \cdot \beta, h_{t-1}^{\text{bd}})\label{eq:gru_bd_2}
\end{align}

\noindent where $t\in [0,N-1]$, $\tau(.)$ is an element-wise step function similarly defined as Eq. (\ref{eq:deterministic_step}), and  $f_{\text{bd}}(\cdot)$ is the boundary detection function, which maps the inputs into a one-dimensional vector by performing a linear transformation. 

The boundary detection mechanism ensures that the input data following a time boundary are not influenced by those seen before the boundary,  and generates a hierarchical representation of the video in which each chunk is composed of homogeneous frames. In our model, we take the final output as the initial input to both the decoders for video captioning and video prediction.



%\noindent\textbf{Boundary-detection based video encoder.}
%Fig.~\ref{fig:bd_video} shows the architecture of $\text{GRU}_{\text{Enc-bd}}$, which consists of two GRU modules, and a boundary-detection network~\cite{baraldi2017hierarchical}.

%Note that when we train the video prediction process, we only use the first 10 frames as the input and the latter 10 frames as the target.

%\noindent\textbf{GRU-based video decoder.}
%The output of encoder in the video captioning which are fit for decoding a suitable word are not corresponding to real elements in the videos because the video captioning model only feeds back information from language decoding process.
%Here, we introduce a visual prediction process into our model to generate a more representative output of encoder from video encoding as Fig. \ref{fig:top}(c) shows.
%our language prediction network is an attention-based network. With additional learning for video information, the video model can get a better understanding of the temporary structure which is helpful for context comprehension.
%Besides, the RNN encoder should extract representative information from the features so that it can predict a reasonable result after the attention model. In this way, the model is forced to learn what are the key elements of the features to keep the main information of the frames.
%The soft attention model is adopted in the video prediction process to evaluate the importance of a frame feature in a prediction process and generate an attention vector from the whole frame features:
%\begin{align}
%g_{\text{att}}(\mathbf{v}_f^{\text{bi}},h_{t-1}^{v})    &=        \sum_{n=0}^{N} \alpha_t^n \odot v^{\text{bi}}_{f_n}\\
%\mathbf{\alpha_t}&= \text{softmax}(\mathbf{W}_{va} \mathbf{A}_{t}+\mathbf{b}_{\alpha})\\
%  A_t^{n}&= \text{tanh}(\mathbf{W}_h^e h_{t-1}^{v}  + \mathbf{W}^e v_{f_n}^{\text{bi}})
%\end{align}
%where $\mathbf{v}_{f}^{\text{bi}}$ is the feature vector and $h_{t-1}^{v}$ is the hidden state from the video decoder. $\alpha_t^n$ are the weights of each frame at time $t$. 
%We use a simple GRU-based decoder noted as $\text{GRU}_{\text{Dec}}^v$ to predict the frame features. Because in this process, a complex predictor is not helpful for the video encoding. A complex RNN predictor can predict a better target feature, but the target features are not directly utilized in video captioning process. Instead, the simple predictor will make video encoding model learn more knowledge to predict the same result in video captioning process.


\subsubsection{Video Prediction}\label{sec:video_prediction}

To learn richer video representations that can  predict the temporal context and actions, we use an alternative (unsupervised) video prediction task %\cite{srivastava15_unsup_video} 
as shown in Figure~\ref{fig:top}(c). The video encoder for this task shares the parameters with the video encoder ($\text{GRU}_{\text{Enc-bi}}^v$) for the caption generation task. 
For each training video, we divide the feature set into 2 subsets $ \{v_{f_0},\cdots, v_{f_{N/2-1}}\}$ and $ \{v_{f_{N/2}},\cdots, v_{f_{N-1}}\}$, which contain same number of contiguous frames.
The first subset is for video encoding, and the second subset is served as ground truth.






%Multi-task learning helps in sharing information between different tasks and across different modalities.
%Our target is to improve the video encoding process.
%Here we introduce an additional video prediction path for this task, see the right part of Figure~\ref{fig:top}.
The prediction of each frame feature is defined as follows:
\begin{align}
%v_{n}^l& = \begin{cases} v_{BD_1} & n=0 \\
%v_{n-1}^{f_2} & \mbox{otherwise} \end{cases}\\
h_{t}^v, o_t^{v} =\text{GRU}_{\text{Dec}}^v \left(g_{\text{att}}(\mathbf{v}^{\text{bi}}, h_{t-1}^{v} ),o_{t-1}^v, h_{t-1}^v \right) \label{eq:20}
\end{align}

\noindent where $h_{t-1}^{v}$ and $o_{t-1}^v$ are the hidden state and the predicted feature at the previous time step, 
 $g_{\text{att}}(\cdot)$ is the attention model which shares the same parameters with Eq.~(\ref{eq:att_0}). We take the final output of $\text{GRU}_{\text{Enc-bd}}^{v}$ as the initial step of the video decoder $\text{GRU}_{\text{Dec}}^v$. 

We train the two related tasks, video captioning and video prediction, jointly in a  multi-task learning framework \cite{luong2015multi}, and demonstrate that the captioning task benefits from incorporating complementary visual knowledge from the video prediction task. 

%$o_t^v$ is the output,  $h_{t-1}^v$ is its hidden state. 



%at each time step, the soft attention model generates a set of weights from the encoded vectors and the hidden state of $\text{GRU}_{\text{Dec}}^v$.
%$o_{t}^{v}$ is the predicted frames features as the linear mapping of $h_t^v$.
%When predicting the next frame feature we usually involve the previous frame we predicted because of the continuity of frames in a video.
%We involve $v_{t}^v$ to express the frame feature at last time step $v_{t-1}^{f_2}$ to apply the continuity in our video prediction. At the beginning of prediction, the prediction model does not receive any information of the previous video.
%Therefore, we pick $v_{BD_1}$, the global vector of all previous frames generated by a Boundary-Detection, as the $v_{0}^l$.
%Then, at each time step, the nearest predicted feature is chosen as the input of $GRU_P$. To simply our training process we use the target video features $v_{n-1}^{f_2}$ to replace the predicted video features $\bar{v}_{n-1}^{f_2}$.
%$g_\text{v}^\text{P}(\cdot)$ and $g_\text{w}^\text{P}(\cdot)$ are the linear mapping functions for $v_{\bar{n}}^{Att_1}$ and $v_{\bar{n}}^{l}$. $\bar{v}_{n}^{f_2}$ is n-th the predicted features for $v^{f_2}$. Due to the different vector sizes of hidden layer $ h_{n}^{\text{P}}$ and $v^{f_2}$.
%We use a linear layer to convert V-dimensional $ h_{n}^{\text{P}}$ to vector K-dimensional $f_t^v$ in the space of $v^{f_2}$. $\mathbf{W}_\text{o}^\text{v} \in R^{K \times V}$ and  $\mathbf{b}_\text{o}^\text{v} \in R^K$ are parameters of linear layer.

\subsection{Training}
%\subsection{Video Captioning Training}
Given the video features $\mathbf{v}_f=(v_{f_0},\cdots, v_{f_{N-1}})$ and the ground-truth caption $(Y_0, Y_1, ..., Y_{T-1})$, the language decoder is conditioned step by step on the first $t$ words of the caption (already generated) and on the corresponding video descriptors in $\mathbf{v}_f$, and is trained to produce the next caption word. We train the caption generation process by minimizing the cross entropy (XE) loss:

\begin{align}
\mathcal{L}_{\text{xe}}=-\sum_{t=0}^{T-1}\log p_{\theta_t}(Y_t|Y_{0:t-1},v_{f_{0:N-1}};\theta)
\label{eq:xe_loss}
\end{align}
where $p_{\theta_t}(Y_t|Y_{0:t-1},v_{f_{0:N-1}})$ is the output probability of the predicted word $Y_t$ with the model parameters $\theta$. We share the weights of the model across all time steps.

For the video prediction path, we optimize the model to minimize the mean squared errors (MSE):
\begin{align}
\mathcal{L}_{\text{MSE}}= \frac{2}{N} \sum_{n=0}^{N/2-1} \|o_n^{v} - v_{f_{N/2+n}}\|^2
\label{eq:mse_loss}
\end{align}
where $v_{f_{N/2+n}}$ serves as the ground truth frame features, and $o_n^{v}$ is the predicted frame features given by the video decoder. 
%When we train the video prediction, the parameters of video predictor GRU will be freeze randomly with the ratio as 0.05 to force the video encoding to learn more knowledge about the videos. We train the two tasks randomly during the training process.

==> experiments-v0.0.tex <==
\section{Experiments}

\subsection{Datasets and Metrics}
\textbf{Microsoft Video Description Corpus (MSVD) \cite{chen2011collecting}.} MSVD contains 2,089 Youtube video clips, 85K English descriptions collected by Amazon Mechanical Turkers.
%The dataset was initially conceived to contain multi-lingual descriptions; however, we only consider captions in the English language.
As done in previous works~\cite{guadarrama2013youtube2text,venugopalan2014translating}, we split the dataset into contiguous groups of videos by index number: 1,200 for training, 100 for validation and 670 for testing. \jf{It doesn't add up to 2089 videos.}

\textbf{MSR-Video to Text (MSR-VTT) \cite{xu2016msr}.} MSR-VTT is a large-scale video description dataset which contains 10K video clips collected from the Internet. These video clips last for 41.2 hours in total, covering the 20 representative categories and diverse visual content collected with 257 queries in the video engines. The dataset contains 200K clip-sentence pairs, and each clip is annotated with about 20 natural sentences. Compared to MSVD, MSR-VTT is more challenging, due to the large variety of videos.

\textbf{Evaluation Metrics}
We use three popular metrics for evaluation:
BLEU~\cite{papineni2002bleu}, METEOR~\cite{denkowski2014meteor}, CIDEr~\cite{vedantam2015cider}.
BLEU is a precision-based metric, calculated by matching the n-grams in candidate and reference captions.
METEOR evaluates the captions by matching n-grams in different forms such as surface, stem and paraphrase found in the generated caption and in references.
CIDEr measures consensus in video descriptions by performing a Term Frequency-Inverse Document Frequency weighting for each n-gram.
% CIDEr is more accurate than BLEU when the number of reference captions is low.

%To ensure a fair evaluation, we use the Microsoft COCO evaluation toolkit\footnote{\url{https://github.com/tylin/coco-caption}} to compute all scores, as done in the previous video captioning works~\cite{yu2015video,pan2015hierarchical}.
\subsection{Implementation Detail}
%\subsubsection{Video Feature Extraction}
We sample 20 video frames at an equal interval for each video.
For each frame, we extract its frame feature with the Resnet101 network pre-trained on ImageNet~\cite{deng2009imagenet}.
We set the dimensionality of the frame features as 2048.

For the preprocessing of captions, we transform all letters in the captions to lowercase.
The corpus of the dataset contains many captions with variable lengths. The total time step needed for training depends on the longest sentence, and it affects the optimized process and the training time. For MSVD, we truncate all captions longer than 10 tokens.
For MSR-VTT, we set the maximum number of words to 15. At the end of a sentence, we add an end-of-sentence tag <EOS>. For a sentence shorter the maximum length, we fill <pad> signals in the elements with indexes larger than that of <EOS>.

During training, we use Adam \cite{kingma2014adam} to train our model. The learning rate is set to $1\times10^{-4}$.
We apply the greedy decoding in our training with a scheduled sampling ratio increasing from 0.0 to 0.125 by 0.025 at every 20 epochs.
The decay parameters are set as $\beta_1 = 0.9$ and $\beta_2 = 0.99$.
We incorporate a simple but efficient dropout layer following the RNN cells with a dropout rate of 0.5.
We add a beginning-of-sentence signal <BOS> as the initial word to start the language generation.
When a sentence reaches the end, <EOS> appears.

During testing, we also consider using beam search in our model. Beam search is the method that iteratively keeps the set of the $k$ best word sequences generated at time step $t$ as the candidates to generate next words. In our experiments, we find that when the beam size is six, our model gets the best performance in general. Particularly, we input <BOS> into the language decoder to start generating video descriptions. At each step, we choose the word with the maximum probability after softmax until we reach <EOS>.




\subsection{Baselines for Comparisons}
To get the insights, we consider the following variants of our method.
For a fair comparison, the output dimension of all hidden states are fixed to 512.

\textbf{BI:}
This is the simplest baseline, as described in Section~\ref{sec:baseline}, which is a conventional encoder-decoder video captioning model. Particularly, we use a bidirectional GRU as the video encoder and a one-layer GRU as the language decoder. This model is trained using Eq.~\eqref{eq:xe_loss}.
%implement the simple encoder-decoder network and add different components step by step to prove the efficiency. Shown as below, we use abbreviations to represent different components. \textbf{BI} is the baseline introduced in Section 3.1. \textbf{BD} is the Boundary Detection encoder. \textbf{SA} is the soft attention model. \textbf{VP} is the video prediction model. \textbf{HLM} is the hierarchical language model.

\textbf{BI + BD + SA:} This baseline use the same bidirectional GRU video encoder as BI, but with an additional boundary detection module (BD) and an attention module (SA).
%We implement an Boundary Detection encoder we introduced in Section 3.2.2, a soft attention model based on the baseline. Before training, we initialize the hidden layer of $\text{GRU}_{\text{Enc-bd}}^v$, $\text{GRU}_{\text{Enc-bi}}^v$ and GRU decoder with zeros.
For each time step, the sentence decoder $\text{GRU}_{\text{Dec}}^l$ predicts the next word based on the previous word and the attended frame features calculated by Eq.~\eqref{eq:att_0}.
Here, we initialize the hidden state of $\text{GRU}_{\text{Dec}}^l$ with the last output of $\text{GRU}_{\text{Enc-bd}}^v$.
We optimize this model using Eq.~\eqref{eq:xe_loss}.

\textbf{BI + BD + SA + VP:} This baseline introduces a video prediction (VP) process to BI+BD+SA.
The video encoder and the attention module of the video prediction path are shared with the video captioning process. We use the video decoder $\text{GRU}_{\text{Dec}}^v$ introduced in Section~\ref{sec:video_prediction}.
All hidden states are initialized with zeros, except the hidden state of $\text{GRU}_{\text{Dec}}^l$.
%We initialize the all the hidden layers with zeros. When we train the video captioning process, we still use the whole video features as input.
%Before training the video prediction process, we divide the video frames into two parts, one is for video encoding, and another is served as ground truth in video prediction. Specifically, for each training video, we divide the set into 2 sets $\{{f_0},\cdots, {f_{N/2-1}}\}$ and $\{{f_{N/2}},\cdots, {f_{N-1}}\}$, which contain same number of contiguous frames. During the video prediction training, the video encoding network encodes the features in the first set. And the $\text{GRU}_{\text{Dec}}^v$ predict the features in the second set one by one as the Eq. (\ref{eq:20}).
%During the training, There is a certain possibility for the model to train the video prediction with a batch.
We optimize the two prediction processes alternatively according to the scheduled probability.
Particularly, in our experiments, we find that 0.5 is the best probability for the model performance because it can make the model learn the knowledge in the video side and the language side evenly.
During the video prediction training process, we freeze $\text{GRU}_{\text{Dec}}^l$, and optimize the network with Eq.~\eqref{eq:mse_loss}.
Similarly, we freeze the parameters of $\text{GRU}_{\text{Dec}}^v$ during the caption prediction process, and optimize the model with Eq.~\eqref{eq:xe_loss}.

\textbf{BI +BD + SA + VP + HLM:} This is the complete set of our method including all the components, where we improve the language decoder $\text{GRU}_{\text{Dec}}^l$ with a hierarchical language model (HLM). Here, the word decoder $\text{B-GRU}$ predicts the next word based on the previous word and the attended frame features as well as the hidden state of the global language model $\text{GRU}_{\text{Dec}}^l$. Different from BI+BD+SA+VP, the soft attention model here also takes in the output of $\text{GRU}_{\text{Dec}}^l$ instead of that of $\text{B-GRU}$. For this final model, we also consider using beam search during testing. For differentiation, we denote our method with and without beam search as BI +BD + SA + VP + HLM and BI +BD + SA + VP + HLM', respectively.
%Then, we keep the video prediction process unchanged and apply the hierarchical language model to replace the GRU decoder used in the video captioning process in Section 4.4.2.
%The detail about the hierarchical language model is introduced in Section~\ref{sec:hlm}.



\subsection{Quantitative Results}
Table~\ref{tab:msvd} shows the comparison results of different baselines and the state-of-the-art methods on the MSVD dataset. Comparing among different baselines of our method, we can see that adding each additional component (including BD, SA, VP and HLM) further improves the performance, which demonstrates the effectiveness of each individual component. Our final model with beam search, \textbf{BI + BD + SA + VP + HLM}, achieves the best performance in all the baselines across all metrics. Compare with the other approaches trained with the single training dataset, our final model achieves the state-of-the-art performance in BLEU 4 and CIDEr Score. Table~\ref{tab:msr-vtt} also lists a few other methods that report better results, but all of them make use of multiple datasets for training.
Table~\ref{tab:msr-vtt} shows the video captioning results of different methods on the MSR-VTT dataset. We can see that our final model can still achieve competitive performance, compared with the state-of-the-art methods.

\begin{table}%[htbp]
	\begin{center}
		\small
	\caption{Comparisons of the video captioning results of different methods on the MSVD dataset.} 	\label{tab:msvd}
		\begin{tabular}{lp{1cm}p{1cm}p{1cm}} %{l|c|c|c}
			\hline
			Model                                                                                 & BLEU 4     & METEOR         & CIDEr         \\
			\hline
\multicolumn{4}{c}{Training with single dataset}\\
			\hline
			MM-VDN~\cite{xu2015multi}    & 34.0    & 29.0    & -            \\
			SA-GoogleNet+3D-CNN\cite{yao2015describing}    & 41.9    & 29.6    & -            \\
			%LSTM-YT\cite{venugopalan2014translating}     & 33.3    & 29.1     & -         \\
			S2VT\cite{venugopalan2015sequence}    & -        & 29.8    & -         \\
			LSTM-E\cite{pan2016jointly}    & 45.3    & 31.0    & -         \\
			Boundary-aware encoder\cite{baraldi2017hierarchical}    & 42.5    & 32.4     & 63.5         \\
			%MA-LSTM~    & 52.3    & \textbf{33.6}    & 70.4     \\
			HRNE\cite{pan2016hierarchical}    & 44.8    & 33.1    & -     \\
			TDDF(VGG+C3D)\cite{zhang122017task}   &45.8   &\textbf{33.3}   &73.0\\
			\hline
			\textbf{BI}				& 35.9	  &		 26.0	 & 56.9\\
			\textbf{BI + BD + SA}        & 37.2    &      27.4    & 63.5        \\
			\textbf{BI + BD + SA + VP}        & 39.6    &      29.1    & 68.1        \\
			\textbf{BI + BD + SA + VP + HLM'}     & 42.7 & 31.6    &71.8         \\
			\textbf{BI + BD + SA + VP + HLM}    & \textbf{50.3} & 32.9    &\textbf{74.3}         \\
			\hline
			\multicolumn{4}{c}{Training with multi-datasets}\\
			\hline
			Entailment Generation\cite{pasunuru2017multi}   &\textbf{54.5}   &\textbf{36.0}   &\textbf{92.4}\\
			SCN-LSTM\cite{gan2017semantic}    &51.1   &33.5   &77.7\\
			$\text{LSTM-TSA}_\text{IV}$~\cite{pan2017video}    & 52.8    & 33.5    & 74.0     \\
			\hline
		\end{tabular}
	\end{center}
\end{table}

\begin{table}%[htbp]
	\begin{center}
		\small
	\caption{Comparisons of the video captioning results of different methods on the MSR-VTT dataset. \jf{It would be better if you could generate the result of our method with beam search.}}
	\label{tab:msr-vtt}
	
		\begin{tabular}{lp{1cm}p{1cm}p{1cm}} %{l|c|c|c}
			\hline
			Model                                                                                 & BLEU 4     & METEOR         & CIDEr \\
			\hline
			%MM-VDN~\cite{xu2015multi}                                        & 37.6    & 29.0    & -            \\
			MP-LSTM(V)\cite{venugopalan2014translating}    & 34.8    & 24.8    & -            \\
			%SA-LSTM(V)\cite{}    & 35.8    & 25.8     & -         \\
			Alto\cite{dong2016early}  &39.2     &29.4   &41.0   \\
			%41.1 27.7 46.4
			MS-RNN(R)\cite{song2017deterministic}    & \textbf{39.8}    & 26.1    & 40.9         \\
			hLSTMt\cite{song2017hierarchical}        & 37.4    & 26.1    & -         \\
			TDDF(VGG+C3D)\cite{zhang122017task}    & 37.3    & \textbf{27.8} & \textbf{43.8}         \\
			\hline
			
			\textbf{BI + BD + SA + VP + HLM'}    & 37.8    & 26.9         &41.3         \\
			\hline
		\end{tabular}
	\end{center}
\end{table}

In our model, we share the soft attention module between the video features and the language features, while a common way is to use two different attention modules. To evaluate the effectiveness of the shared attention module, we train our baseline of \textbf{BI + BD + SA + VP} with the two different attention mechanisms, whose testing results are shown in Table~\ref{tab:SA}. It can be seen that the proposed shared attention module achieves better performance.

\begin{table}%[tbhp]
	\begin{center}
		\small
	\caption{Comparisons of the video captioning results of our baseline of \textbf{BI + BD + SA + VP} with different soft attention models.}
	\label{tab:SA}
		\begin{tabular}{lp{1cm}p{1cm}p{1cm}} %{l|c|c|c}
			\hline
			Model                                                                                 & BLEU 4     & METEOR         & CIDEr          \\
			\hline
			%MM-VDN~\cite{xu2015multi}                                        & 37.6    & 29.0    & -            \\
			%No-prediction    & 37.2    & 27.4 & 63.5            \\
			%SA-LSTM(V)\cite{}    & 35.8    & 25.8     & -         \\
			Two-attentions  & 38.8    & 28.3 &65.7   \\
			%41.1 27.7 46.4
			Single-attention     & 39.6    & 29.1    & 68.1         \\
			\hline
		\end{tabular}
	\end{center}
\end{table}

\subsection{Qualitative Results}
Figure~\ref{fig:results} gives some examples of the generated captions.
We can see that our model can avoid some mistakes caused by the conventional language decoding.
Taking the first two videos as example, our model can predict much better results compared with the baseline.
%In the third and fourth video, we can see that our model predict a part of correct sentences, and further predicts some correct information which is better than the baseline.
In the fourth video, even though the "dog" is the main object in the video, our model can avoid making the object (e.g, "baby") and the subject (e.g, "dog") to be the same (although our generated caption is also incorrect).
%Our final model can successfully detects "\textcolor{red}{xxx}" in the video and
%The model views the baby as a monkey in the video and distinguishes it from the dog.
%In the sixth video, our model and the baseline provide a poor performance on that.
The cases in the fifth and sixth videos are failure cases, which are mainly due to the highly similar objects in the video. Specifically, in the fifth video, our final model confuses ``running" with ``riding" because many people are running in the street and the people behind seem to be "riding" on the front people. In the sixth video, our model predicts the correct subject "cat" but fails to predict the rest words. It is mainly because the reflection of the floor is similar to water.

Figure \ref{fig:prove} shows the results of the language boundary detection from the binary gate defined in \eqref{eq:deterministic_step}, where a 0 indicates there is no boundary at that position while 1 indicates there is a boundary. We can see that our language boundary detection model can detect the boundary between nouns and verbs. The model considers a sentence as several different word groups such as ``a bowl" and ``on bread". In the first example, that the model considers the word ``the" has a strong dependency with "is playing with" is mainly because the noun after ``the" can change variably, but the word group ``playing with the" has a relatively stable form.

\begin{figure}%[tbhp]
	\centering
	%\begin{minipage}[t]{\linewidth}
	%	\centering
		\includegraphics[width=\linewidth]{prove.png}
		\caption{Examples of the language boundary detection.}
		\label{fig:prove}
	%\end{minipage}
\end{figure}

\begin{figure*}%[tbhp]
	\centering
	%\begin{minipage}[t]{\linewidth}
		%\centering
		\includegraphics[width=\linewidth]{vis_examples.png}
		\caption{Examples of the generated captions by our final model and a baseline.}
		\label{fig:results}
	%\end{minipage}
\end{figure*}



%, we think that such a shared attention mechanism helps the language decoding.




==> experiments-v0.1.tex <==
\section{Experiments}

\subsection{Datasets and Metrics}
\textbf{Microsoft Video Description Corpus (MSVD) \cite{chen2011collecting}.} MSVD contains 1,970 Youtube video clips, 85K English descriptions collected by Amazon Mechanical Turkers.
%The dataset was initially conceived to contain multi-lingual descriptions; however, we only consider captions in the English language.
As done in previous works~\cite{guadarrama2013youtube2text,venugopalan2014translating}, we split the dataset into contiguous groups of videos by index number: 1,200 for training, 100 for validation and 670 for testing. 

\textbf{MSR-Video to Text (MSR-VTT) \cite{xu2016msr}.} MSR-VTT is a large-scale video description dataset which contains 10K video clips collected from the Internet. These video clips last for 41.2 hours in total, covering the 20 representative categories and diverse visual content collected with 257 queries in the video engines. The dataset contains 200K clip-sentence pairs, and each clip is annotated with about 20 natural sentences. Compared to MSVD, MSR-VTT is more challenging, due to the large variety of videos.

\textbf{Evaluation Metrics}
We use three popular metrics for evaluation:
BLEU~\cite{papineni2002bleu}, METEOR~\cite{denkowski2014meteor}, CIDEr~\cite{vedantam2015cider}.
BLEU is a precision-based metric, calculated by matching the n-grams in candidate and reference captions.
METEOR evaluates the captions by matching n-grams in different forms such as surface, stem and paraphrase found in the generated caption and in references.
CIDEr measures consensus in video descriptions by performing a Term Frequency-Inverse Document Frequency weighting for each n-gram.
% CIDEr is more accurate than BLEU when the number of reference captions is low.

%To ensure a fair evaluation, we use the Microsoft COCO evaluation toolkit\footnote{\url{https://github.com/tylin/coco-caption}} to compute all scores, as done in the previous video captioning works~\cite{yu2015video,pan2015hierarchical}.
\subsection{Implementation Detail}
%\subsubsection{Video Feature Extraction}
We sample 20 video frames at an equal interval for each video.
For each frame, we extract its frame feature with the Resnet101 network pre-trained on ImageNet~\cite{deng2009imagenet}.
We set the dimensionality of the frame features as 2,048.

For the preprocessing of captions, we transform all letters in the captions to lowercase.
The corpus of the dataset contains many captions with variable lengths. The total time step needed for training depends on the longest sentence, and it affects the optimized process and the training time. For MSVD, we truncate all captions longer than 10 tokens.
For MSR-VTT, we set the maximum number of words to 15. At the end of a sentence, we add an end-of-sentence tag <EOS>. For a sentence shorter the maximum length, we fill <pad> signals in the elements with indexes larger than that of <EOS>.

During training, we use Adam \cite{kingma2014adam} to train our model. The learning rate is set to $1\times10^{-4}$.
We apply the greedy decoding in our training with a scheduled sampling ratio increasing from 0.0 to 0.125 by 0.025 at every 20 epochs.
The decay parameters are set as $\beta_1 = 0.9$ and $\beta_2 = 0.99$.
We incorporate a simple but efficient dropout layer following the RNN cells with a dropout rate of 0.5.
We add a beginning-of-sentence signal <BOS> as the initial word to start the language generation.
When a sentence reaches the end, <EOS> appears.

During testing, we also consider using beam search in our model. Beam search is the method that iteratively keeps the set of the $k$ best word sequences generated at time step $t$ as the candidates to generate next words. In our experiments, we find that when the beam size is six, our model gets the best performance in general. Particularly, we input <BOS> into the language decoder to start generating video descriptions. At each step, we choose the word with the maximum probability after softmax until we reach <EOS>.




\subsection{Baselines for Comparisons}
To get the insights, we consider the following variants of our method.
For a fair comparison, the output dimension of all hidden states are fixed to 512.

\textbf{BI:}
This is the simplest baseline, as described in Section~\ref{sec:baseline}, which is a conventional encoder-decoder video captioning model. Particularly, we use a bidirectional GRU as the video encoder and a one-layer GRU as the language decoder. This model is trained using Eq.~\eqref{eq:xe_loss}.
%implement the simple encoder-decoder network and add different components step by step to prove the efficiency. Shown as below, we use abbreviations to represent different components. \textbf{BI} is the baseline introduced in Section 3.1. \textbf{BD} is the Boundary Detection encoder. \textbf{SA} is the soft attention model. \textbf{VP} is the video prediction model. \textbf{HLM} is the hierarchical language model.

\textbf{BI + BD + SA:} This baseline use the same bidirectional GRU video encoder as BI, but with an additional boundary detection module (BD) and an attention module (SA).
%We implement an Boundary Detection encoder we introduced in Section 3.2.2, a soft attention model based on the baseline. Before training, we initialize the hidden layer of $\text{GRU}_{\text{Enc-bd}}^v$, $\text{GRU}_{\text{Enc-bi}}^v$ and GRU decoder with zeros.
For each time step, the sentence decoder $\text{GRU}_{\text{Dec}}^l$ predicts the next word based on the previous word and the attended frame features calculated by Eq.~\eqref{eq:att_0}.
Here, we initialize the hidden state of $\text{GRU}_{\text{Dec}}^l$ with the last output of $\text{GRU}_{\text{Enc-bd}}^v$.
We optimize this model using Eq.~\eqref{eq:xe_loss}.

\textbf{BI + BD + SA + VP:} This baseline introduces a video prediction (VP) process to BI+BD+SA.
The video encoder and the attention module of the video prediction path are shared with the video captioning process. We use the video decoder $\text{GRU}_{\text{Dec}}^v$ introduced in Section~\ref{sec:video_prediction}.
All hidden states are initialized with zeros, except the hidden state of $\text{GRU}_{\text{Dec}}^l$.
%We initialize the all the hidden layers with zeros. When we train the video captioning process, we still use the whole video features as input.
%Before training the video prediction process, we divide the video frames into two parts, one is for video encoding, and another is served as ground truth in video prediction. Specifically, for each training video, we divide the set into 2 sets $\{{f_0},\cdots, {f_{N/2-1}}\}$ and $\{{f_{N/2}},\cdots, {f_{N-1}}\}$, which contain same number of contiguous frames. During the video prediction training, the video encoding network encodes the features in the first set. And the $\text{GRU}_{\text{Dec}}^v$ predict the features in the second set one by one as the Eq. (\ref{eq:20}).
%During the training, There is a certain possibility for the model to train the video prediction with a batch.
We optimize the two prediction processes alternatively according to the scheduled probability.
Particularly, in our experiments, we find that 0.5 is the best probability for the model performance because it can make the model learn the knowledge in the video side and the language side evenly.
During the video prediction training process, we freeze $\text{GRU}_{\text{Dec}}^l$, and optimize the network with Eq.~\eqref{eq:mse_loss}.
Similarly, we freeze the parameters of $\text{GRU}_{\text{Dec}}^v$ during the caption prediction process, and optimize the model with Eq.~\eqref{eq:xe_loss}.

\textbf{BI +BD + SA + VP + HLM:} This is the complete set of our method including all the components, where we improve the language decoder $\text{GRU}_{\text{Dec}}^l$ with a hierarchical language model (HLM). Here, the word decoder $\text{B-GRU}$ predicts the next word based on the previous word and the attended frame features as well as the hidden state of the global language model $\text{GRU}_{\text{Dec}}^l$. Different from BI+BD+SA+VP, the soft attention model here also takes in the output of $\text{GRU}_{\text{Dec}}^l$ instead of that of $\text{B-GRU}$. For this final model, we also consider using beam search during testing.
%For differentiation, we denote our method with and without beam search as BI +BD + SA + VP + HLM and BI +BD + SA + VP + HLM$'$, respectively.
%Then, we keep the video prediction process unchanged and apply the hierarchical language model to replace the GRU decoder used in the video captioning process in Section 4.4.2.
%The detail about the hierarchical language model is introduced in Section~\ref{sec:hlm}.



\subsection{Quantitative Results}
Table~\ref{tab:msvd} shows the comparison results of different baselines and the state-of-the-art methods on the MSVD dataset. Comparing among different baselines of our method, we can see that adding each additional component (including BD, SA, VP and HLM) further improves the performance, which demonstrates the effectiveness of each individual component. 
%
In our model, we share the soft attention module between the video features and the language features, while a common way is to use two different attention modules. To evaluate the effectiveness of the shared attention module, we train our baseline of \textbf{BI + BD + SA + VP} with the two different attention mechanisms, whose testing results are shown in Table~\ref{tab:msvd}. It can be seen that the proposed shared attention module achieves better performance.
Our final model with beam search, \textbf{BI + BD + SA + VP + HLM}, achieves the best performance in all the baselines across all metrics. Compare with the other approaches trained with the single training dataset, our final model achieves the state-of-the-art performance in BLEU 4 and CIDEr Score.


Table~\ref{tab:msr-vtt} also lists a few other methods that report better results, but all of them make use of multiple datasets for training.
Table~\ref{tab:msr-vtt} shows the video captioning results of different methods on the MSR-VTT dataset. We can see that our final model can still achieve competitive performance, compared with the state-of-the-art methods.

\begin{table}%[htbp]
	\begin{center}
		\small
	\caption{Comparisons of the video captioning results of different methods on the MSVD dataset.} 	\label{tab:msvd}
		\begin{tabular}{lp{1cm}p{1cm}p{1cm}} %{l|c|c|c}
			\hline
			Model                                                                                 & BLEU 4     & METEOR         & CIDEr         \\
			\hline
\multicolumn{4}{c}{Training with single dataset}\\
			\hline
			MM-VDN~\cite{xu2015multi}    & 34.0    & 29.0    & -            \\
			SA-GoogleNet+3D-CNN\cite{yao2015describing}    & 41.9    & 29.6    & -            \\
			%LSTM-YT\cite{venugopalan2014translating}     & 33.3    & 29.1     & -         \\
			S2VT\cite{venugopalan2015sequence}    & -        & 29.8    & -         \\
			LSTM-E\cite{pan2016jointly}    & 45.3    & 31.0    & -         \\
			Boundary-aware encoder\cite{baraldi2017hierarchical}    & 42.5    & 32.4     & 63.5         \\
			%MA-LSTM~    & 52.3    & \textbf{33.6}    & 70.4     \\
			HRNE\cite{pan2016hierarchical}    & 44.8    & 33.1    & -     \\
			TDDF(VGG+C3D)\cite{zhang122017task}   &45.8   &\textbf{33.3}   &73.0\\
			\hline
			\textbf{BI} (greedy)				& 35.9	  &		 26.0	 & 56.9\\
			\textbf{BI + BD + SA} (greedy)        & 37.2    &      27.4    & 63.5        \\
			\textbf{BI + BD + $\text{SA}^{*}$ + VP} (greedy)& 38.8    & 28.3 &65.7 \\
			\textbf{BI + BD + SA + VP} (greedy)        & 39.6    &      29.1    & 68.1        \\
			
			\textbf{BI + BD + SA + VP + HLM} (greedy)     & 42.7 & 31.6    &71.8         \\
			\textbf{BI + BD + SA + VP + HLM} (beam)    & \textbf{50.3} & 32.9    &\textbf{74.3}         \\
			\hline
			\multicolumn{4}{c}{Training with multi-datasets}\\
			\hline
			Entailment Generation\cite{pasunuru2017multi}   &\textbf{54.5}   &\textbf{36.0}   &\textbf{92.4}\\
			SCN-LSTM\cite{gan2017semantic}    &51.1   &33.5   &77.7\\
			$\text{LSTM-TSA}_\text{IV}$~\cite{pan2017video}    & 52.8    & 33.5    & 74.0     \\
			\hline
		\end{tabular}
	\end{center}
\end{table}

\begin{table}%[htbp]
	\begin{center}
		\small
	\caption{Comparisons of the video captioning results of different methods on the MSR-VTT dataset. }
	\label{tab:msr-vtt}
	
		\begin{tabular}{lp{1cm}p{1cm}p{1cm}} %{l|c|c|c}
			\hline
			Model                                                                                 & BLEU 4     & METEOR         & CIDEr \\
			\hline
			%MM-VDN~\cite{xu2015multi}                                        & 37.6    & 29.0    & -            \\
			MP-LSTM(V)\cite{venugopalan2014translating}    & 34.8    & 24.8    & -            \\
			%SA-LSTM(V)\cite{}    & 35.8    & 25.8     & -         \\
			Alto\cite{dong2016early}  &39.2     &29.4   &41.0   \\
			%41.1 27.7 46.4
			MS-RNN(R)\cite{song2017deterministic}    & \textbf{39.8}    & 26.1    & 40.9         \\
			hLSTMt\cite{song2017hierarchical}        & 37.4    & 26.1    & -         \\
			TDDF(VGG+C3D)\cite{zhang122017task}    & 37.3    & \textbf{27.8} & \textbf{43.8}         \\
			\hline
			
			\textbf{BI + BD + SA + VP + HLM} (beam)    & \textbf{39.8}    & 26.4         &43.3         \\
			\hline
		\end{tabular}
	\end{center}
\end{table}


\begin{figure*}[tb!]
	\centering
	%\begin{minipage}[t]{\linewidth}
	%\centering
	\includegraphics[width=\linewidth]{vis_examples.png}
	\caption{Examples of the generated captions by our final model and a baseline.}
	\label{fig:results}
	%\end{minipage}
\end{figure*}

\subsection{Qualitative Results}
Figure~\ref{fig:results} gives some examples of the generated captions.
We can see that our model can avoid some mistakes caused by the conventional language decoding.
Taking the first two videos as example, our model can predict much better results compared with the baseline.
%In the third and fourth video, we can see that our model predict a part of correct sentences, and further predicts some correct information which is better than the baseline.
In the fourth video, even though the "dog" is the main object in the video, our model can avoid making the object (e.g, "baby") and the subject (e.g, "dog") to be the same (although our generated caption is also incorrect).
%Our final model can successfully detects "\textcolor{red}{xxx}" in the video and
%The model views the baby as a monkey in the video and distinguishes it from the dog.
%In the sixth video, our model and the baseline provide a poor performance on that.
The cases in the fifth and sixth videos are failure cases, which are mainly due to the highly similar objects in the video. Specifically, in the fifth video, our final model confuses ``running" with ``riding" because many people are running in the street and the people behind seem to be "riding" on the front people. In the sixth video, our model predicts the correct subject "cat" but fails to predict the rest words. It is mainly because the reflection of the floor is similar to water.

%Figure \ref{fig:prove} shows the results of the language boundary detection from the binary gate defined in \eqref{eq:deterministic_step}, where a 0 indicates there is no boundary at that position while 1 indicates there is a boundary. We can see that our language boundary detection model can detect the boundary between nouns and verbs. The model considers a sentence as several different word groups such as ``a bowl" and ``on bread". In the first example, that the model considers the word ``the" has a strong dependency with "is playing with" is mainly because the noun after ``the" can change variably, but the word group ``playing with the" has a relatively stable form.



%, we think that such a shared attention mechanism helps the language decoding.




==> experiments2.tex <==
\section{Experiments}

\subsection{Datasets}
\subsubsection{Microsoft Video Description Corpus (MSVD)}~The Microsoft Video Description Corpus~\cite{chen2011collecting} contains 2,089 Youtube video clips, 85K English descriptions collected by Amazon Mechanical Turkers.
%The dataset was initially conceived to contain multi-lingual descriptions; however, we only consider captions in the English language. 
As done in previous works~\cite{guadarrama2013youtube2text,venugopalan2014translating}, we split the dataset into contiguous groups of videos by index number: 1,200 for training, 100 for validation and 670 for testing. 

\subsubsection{MSR-Video to Text (MSR-VTT)}~MSR-Video-to-Text~\cite{xu2016msr} is a large-scale video description dataset which contains 10K video clips collected from the Internet.
%Those video clips last 41.2 hours in total, covering the 20 representative categories and diverse visual content collected with 257 queries in the video engines. 
The dataset contains 200K clip-sentence pairs, and each clip is annotated with about 20 natural sentences. Compared to MSVD, MSR-VTT is more challenging, due to the high variety of video and relatively fewer captions for each video.

\subsection{Metrics}
We employ four popular metrics for evaluation: 
BLEU~\cite{papineni2002bleu}, METEOR~\cite{denkowski2014meteor}, CIDEr~\cite{vedantam2015cider}.
BLEU is a precision-based metric. It is calculated by matching the n-grams in candidate and reference captions.
METEOR computes the average cosine similarity between n-grams found in the generated caption and those found in reference sentences.
CIDEr measures consensus in video descriptions by performing a Term Frequency-Inverse Document Frequency weighting for each n-gram. CIDEr is more accurate than BLEU when the number of reference captions is low.

%To ensure a fair evaluation, we use the Microsoft COCO evaluation toolkit\footnote{\url{https://github.com/tylin/coco-caption}} to compute all scores, as done in the previous video captioning works~\cite{yu2015video,pan2015hierarchical}.
\subsection{Preprocessing}
%\subsubsection{Video Feature Extraction} 
We extract the 20 video frames at the equal interval for each video.
For each frame, we extract the frame features with the Resnet101 network pre-trained on ImageNet~\cite{deng2009imagenet}.
We set the dimensionality of the frame features as 2048.
%\subsubsection{Captions preprocessing} 
As for preprocessing of captions, we transform all letters in the captions to lowercase.
%The corpus of the dataset contains many captions with variant lengths. The total time step needed for training depends on the longest sentences in the batch. A too long sentence in the batch will cause bringing pads following the end signal of short sentences. It will influence the optimized process and enlarge the training time. 
For MSVD, we truncate all captions longer than 10 tokens.
For MSR-VTT we set the maximum number of words to 15.
%set the max length of a caption as 10 words. When a caption is longer than 10 words, we drop the excess words in the caption to make it contains 10 words at maximum. Similar to preprocess of MSVD, we set the max length of captions in MSR-VTT as 15 words and perform same actions. 

%\subsubsection{Training and testing}
%During training, the number $N$ of frames taken from a video equal to 20. They are divided into 2 parts with 10 frames in each set. The model encodes the former 10 frames with same video encoder and attention model of video captioning, and predict the latter 10 frames with a GRU decoder. During the training, we lock the parameter of the decoder at a certain ratio to force the attention and encoding parts to learn more information. 


During the training, we use Adam\cite{kingma2014adam} to train our model. the learning rate we choose is $1\times10^{-4}$. 
We apply the greedy decoding in our training. %The ratio increase from 0.0 to 0.125 by 0.025 at every 20 epochs.
During testing, we apply the beam search in our model. Beam search is the method that iteratively keeps the set of the k best word sequences generated recently t as candidates to generate next words. From all the results, the model keeps only the best k of them for the further generation. %During the testing, the model gets the best performance when the beam size is 6.

\subsection{Models for Comparison}
To get the insight view of our method, we compare our final approach with various baseline approaches.
For a fair comparison, the output dimension of all hidden states are fixed to 512.

\subsubsection{BI}
We first implement an encoder-decoder video captioning model which adopts a bidirectional GRU as video encoder and one-layer GRU as decoder. Here, the pre-trained ResNet101 is adopted as the frame encoder. This model is trained using Eq.\eqref{eq:xe_loss}.
%implement the simple encoder-decoder network and add different components step by step to prove the efficiency. Shown as below, we use abbreviations to represent different components. \textbf{BI} is the baseline introduced in Section 3.1. \textbf{BD} is the Boundary Detection encoder. \textbf{SA} is the soft attention model. \textbf{VP} is the video prediction model. \textbf{HLM} is the hierarchical language model.

\subsubsection{BI + BD + SA} This baseline use the same bidirectional GRU video encoders as BI, but with a additional boundary detection module and an attention module.  
%We implement an Boundary Detection encoder we introduced in Section 3.2.2, a soft attention model based on the baseline. Before training, we initialize the hidden layer of $\text{GRU}_{\text{Enc-bd}}^v$, $\text{GRU}_{\text{Enc-bi}}^v$ and GRU decoder with zeros. 
For each time step, the sentence decoder $\text{GRU}_{\text{Dec}}^l$ predicts the next word based on the previous word and the attended frame features calculated by Eq.~\eqref{eq:att_0}.
Here, we initialize the hidden state of $\text{GRU}_{\text{Dec}}^l$ with the last output of $\text{GRU}_{\text{Enc-bd}}^v$.
We optimize this model with Eq.\eqref{eq:xe_loss}.

\subsubsection{BI +BD + SA + VP} This baseline introduces a video prediction process to BI+BD+SA.
The video encoder and attention module of the video prediction path are shared with video captioning process. We apply $\text{GRU}_{\text{Dec}}^v$ introduced in Section~\ref{sec:video_prediction} as the video decoder.
All hidden state are initialized with zeros, except the hidden of $\text{GRU}_{\text{Dec}}^l$.
%We initialize the all the hidden layers with zeros. When we train the video captioning process, we still use the whole video features as input.
%Before training the video prediction process, we divide the video frames into two parts, one is for video encoding, and another is served as ground truth in video prediction. Specifically, for each training video, we divide the set into 2 sets $\{{f_0},\cdots, {f_{N/2-1}}\}$ and $\{{f_{N/2}},\cdots, {f_{N-1}}\}$, which contain same number of contiguous frames. During the video prediction training, the video encoding network encodes the features in the first set. And the $\text{GRU}_{\text{Dec}}^v$ predict the features in the second set one by one as the Eq. (\ref{eq:20}). 
%During the training, There is a certain possibility for the model to train the video prediction with a batch. 
We optimize the two prediction processes sequentially according to scheduled probability.
And in our experiments, we find that 0.5 is the best for the model performance because it can make the model learn the knowledge in video and language side evenly.
During the video prediction training process, we freeze the sentence decoders $\text{GRU}_{\text{Dec}}^l$ and $\text{B-GRU}$. We only optimize the network with Eq.~\eqref{eq:mse_loss}.
Similarly, we freeze the parameter of $\text{GRU}_{\text{Dec}}^v$ during the caption prediction process, and optimize the model with Eq.~\eqref{eq:xe_loss}.

\subsubsection{BI +BD + SA + VP + HLM} This baseline improves the $\text{GRU}_{\text{Dec}}^l$ with a hierarchical language model.
%Then, we keep the video prediction process unchanged and apply the hierarchical language model to replace the GRU decoder used in the video captioning process in Section 4.4.2. 
%The detail about the hierarchical language model is introduced in Section~\ref{sec:hlm}. 
Before video captioning training, we initialize the hidden state of $\text{GRU}_{\text{Dec}}^l$ with the final output of boundary detection encoder $\text{GRU}_{\text{Enc-bd}}^v$.
%The initialization of video prediction is same as the that in Section 4.4.2. 
The whole frame features are sent to the $\text{GRU}_{\text{Enc-bi}}^v$ to generate a set of encoded features.
The encoded features are utilized by soft attention model to generate an attention vector. Different from BI+BD+SA+VP, another input of the soft attention model is the output of the $\text{GRU}_{\text{Dec}}^l$ instead of the output of $\text{B-GRU}$.
%With the attention vector, the B-GRU generate words following the equations from Eq.~\eqref{eq:9}) to Eq. (14). 
%Note that the hidden size of the hierarchical language model is also 512. Specially, since B-GRU input is the join of $v^att_t$, $y_{t-1}$ and $h_t^l$, the size of it is 1536 instead of 512.
%The size of hidden layer in our model is 512. 
\section{Analysis}
\begin{figure*}[tbhp]
	\centering
	\begin{minipage}[t]{\linewidth}
		\centering
		\includegraphics[width=\linewidth]{vis_examples.png}
		\caption{Results comparison between our results and baseline.}
		\label{fig:results}
	\end{minipage}
\end{figure*}
\subsection{Quantity Analysis}
In Table~\ref{tab:msvd}, we compare our methods with the state-of-the-art methods on MSVD.
{BI} is our baseline model with a bidirectional GRU as video encoder.
After introducing attention mechanism and boundary-aware video encode, we can see that {BI+BD+SA} performs better than {BI}.
%Our baseline is the encoder-decoder structure with a bi-direction GRU shown as \textbf{BI}. Firstly, we complete the model combined with the \textbf{BD} and \textbf{SA}. Then we add the video prediction task \textbf{VP} into our training process shown as BD+SA+VP in Tab. \ref{tab:msvd}. 
We also observe that video prediction can significantly im-prove the performance of video captioning.
%After adding the video prediction path, we achieve better performance compared with 
This illustrates that the video prediction task can help our model to learn a more powerful video encoder and soft attention model.
After incorporating  hierarchical language model,  our  BI+BD+SA + VP + HLM model shows significant improvements across all metrics.
Note that we perform the beam search for our final model.
%into our model to guide the video soft attention. Compared with the former model, $\text{GRU}_{\text{Dec}}^l$ improves all the scores tested. Finally, the beam search (beam) is used in the final evaluation shown as BD+SA+VP+
%a HLM(beam) in Tab. \ref{tab:msvd}. The detail of the complementation is shown in Section 4.4.
%Scores of our model tested on MSVD and MSR-VTT are shown in Tab. \ref{tab:msvd} and Tab. %\ref{tab:msr-vtt}. In Tab. \ref{tab:msvd}, comparing with the other models trained by single training dataset, our model gets the state-of-the-art position in Bleu 4 and CIDEr Score.  
We also evaluate our model on MSR-VTT.
Table~\ref{tab:msr-vtt} shows the performance comparisons on MSR-VTT.
We can see hat our final model can still achieves the comparable performance compared with the state-of-the-art methods.

Table~\ref{tab:SA} show the performance comparison with the independent attention mechanism and shared attention mechanism.
We can see that our structure with the shared attention achieves better performance.
%To further illustrate the efficiency of the soft attention shared by video prediction and video captioning process, we test the shared-attention model with the model with 2 independent attention and. The result shows that the shared attention with can generate better results shown as Tab. \ref{tab:SA}:

%, our results in MSR-VTT is not so good as that in MSVD. But our model still keeps close to the state-of-art position.

\begin{table}[htbp]
	\begin{center}
		\small
		\begin{tabular}{lp{1cm}p{1cm}p{1cm}} %{l|c|c|c}
			\hline
			Model                                                                                 & B@4     & M         & C         \\
			\hline
			MM-VDN~\cite{xu2015multi}    & 34.0    & 29.0    & -            \\
			SA-GoogleNet+3D-CNN\cite{yao2015describing}    & 41.9    & 29.6    & -            \\
			%LSTM-YT\cite{venugopalan2014translating}     & 33.3    & 29.1     & -         \\
			S2VT\cite{venugopalan2015sequence}    & -        & 29.8    & -         \\
			LSTM-E\cite{pan2016jointly}    & 45.3    & 31.0    & -         \\
			Boundary-aware encoder\cite{baraldi2017hierarchical}    & 42.5    & 32.4     & 63.5         \\
			%MA-LSTM~    & 52.3    & \textbf{33.6}    & 70.4     \\            
			HRNE\cite{pan2016hierarchical}    & 44.8    & 33.1    & -     \\
			TDDF(VGG+C3D)\cite{zhang122017task}   &45.8   &33.3   &73.0\\
			\hline
			\textbf{BI}				& 35.9	  &		 26.0	 & 56.9\\
			\textbf{BD + SA}        & 37.2    &      27.4    & 63.5        \\
			\textbf{BD + SA + VP}        & 39.6    &      29.1    & 68.1        \\
			%BD + SA + VP + FR     & 42.7 & 31.6    &71.8         \\
			\textbf{BD + SA + VP + HLM (beam)}    & \textbf{50.3} & 32.9    &\textbf{74.3}         \\
			\hline
			The model training with multi-datasets\\
			\hline
			Entailment Generation\cite{pasunuru2017multi}   &\textbf{54.5}   &\textbf{36.0}   &\textbf{92.4}\\
			SCN-LSTM\cite{gan2017semantic}    &51.1   &33.5   &77.7\\
			$\text{LSTM-TSA}_\text{IV}$~\cite{pan2017video}    & 52.8    & 33.5    & 74.0     \\
			\hline
		\end{tabular}
	\end{center}
	\caption{Experiment results on the MSVD dataset.}
	\label{tab:msvd}
	
\end{table}

%\begin{table}[htbp]
%	\begin{center}
%		\small
%		\begin{tabular}{lp{1cm}p{1cm}p{1cm}} %{l|c|c|c}
%			\hline
%			Model                                                                                 & B@4     & M         & C         \\
%			The model training with multi-datasets\\
%			\hline
%			Entailment Generation\cite{pasunuru2017multi}   &\textbf{54.5}   &\textbf{36.0}   &\textbf{92.4}\\
%			SCN-LSTM\cite{gan2017semantic}    &51.1   &33.5   &77.7\\
%			$\text{LSTM-TSA}_\text{IV}$~\cite{pan2017video}    & 52.8    & 33.5    & 74.0     \\
%			\hline
%			BD + SA + VP + HLM (beam)    & \textbf{50.3} & 32.9    &\textbf{74.3}         \\
%			\hline
%		\end{tabular}
%	\end{center}
%	\caption{Experiment results on the MSVD dataset.}
%	\label{tab:msvd}

%\end{table}



\begin{table}[htbp]
	\begin{center}
		\small
		\begin{tabular}{lp{1cm}p{1cm}p{1cm}} %{l|c|c|c}
			\hline
			Model                                                                                 & B@4     & M         & C         \\
			\hline
			%MM-VDN~\cite{xu2015multi}                                        & 37.6    & 29.0    & -            \\
			MP-LSTM(V)\cite{venugopalan2014translating}    & 34.8    & 24.8    & -            \\
			%SA-LSTM(V)\cite{}    & 35.8    & 25.8     & -         \\
			Alto\cite{dong2016early}  &39.2     &29.4   &41.0   \\
			%41.1 27.7 46.4
			MS-RNN(R)\cite{song2017deterministic}    & \textbf{39.8}    & 26.1    & 40.9         \\
			hLSTMt\cite{song2017hierarchical}        & 37.4    & 26.1    & -         \\
			TDDF(VGG+C3D)\cite{zhang122017task}    & 37.3    & \textbf{27.8} & \textbf{43.8}         \\
			\hline
			
			\textbf{BD + SA + VP + HLM}    & 37.8    & 26.9         &41.3         \\
			\hline
		\end{tabular}
	\end{center}
	\caption{Experiment results on the MSR-VTT dataset.}
	\label{tab:msr-vtt}
	
\end{table}


\begin{table}[tbhp]
	\begin{center}
		\small
		\begin{tabular}{lp{1cm}p{1cm}p{1cm}} %{l|c|c|c}
			\hline
			Model   & B@4     & M     & C         \\
			\hline
			%MM-VDN~\cite{xu2015multi}                                        & 37.6    & 29.0    & -            \\
			%No-prediction    & 37.2    & 27.4 & 63.5            \\
			%SA-LSTM(V)\cite{}    & 35.8    & 25.8     & -         \\
			Two-attentions  & 38.8    & 28.3 &65.7   \\
			%41.1 27.7 46.4
			Single-attention     & 39.6    & 29.1    & 68.1         \\
			\hline
		\end{tabular}
	\end{center}
	\caption{Experiment results on the different soft attention models.}
	\label{tab:SA}
\end{table}

%The results prove that the model with the prediction is better than the model without a prediction which means the additional video information is helpful for the model to predict captions. 

%, we think that such a shared attention mechanism helps the language decoding.

%\subsubsection{frame relocator}
%In our model, we introduce an enhanced attention model developed from a soft attention model. A frame relocator is applied to generate a guidance for soft attention from the phrases split from sentences.  

%\subsubsection{Classical Soft Attention Model}
\subsection{Quality Analysis}
Figure~\ref{fig:results} shows some generated captions.
We can see that our model can also avoid some mistakes caused by the language decoding.
Take the first two video as example, our model can predict better results compared with the baseline.
%In the third and fourth video, we can see that our model detects a part of correct sentences, and further predicts some correct information which is better than the baseline. 
In the fifth video, even though the "dog" is the main attribute in the video, our model can still avoid considering the object (e.g, "baby" or "monkey") and the subject (e.g, "dog") to be the same.
%Our final model can successfully detects "\textcolor{red}{xxx}" in the video and  
%The model views the baby as a monkey in the video and distinguishes it from the dog. 
%In the sixth video, our model and the baseline provide a poor performance on that. 
As for the third and sixth videos, we think the failure results are due to the highly similar objects in the video.
In the fourth video, our final model confuses "running" with the "riding" due to many people are running in the street that the people behind seems to "riding" on the front people. In the video 6, our model predicted the correct subject "cat" but fail to predict the rest words. It is mainly because that reflection of the floor is similar to the water.

==> releated_works_SHI.tex <==
\section{Related Work}
%\subsubsection{Template-based captioning:}
The problem of video captioning is a hot topic in computer vision and natural language processing communities.
Prior to using deep neural networks for generating video descriptions, the classical approach is to treat the problem as a template-based problem.
Early works in video captioning~\cite{guadarrama2013youtube2text,krishnamoorthy2013generating,thomason2014integrating} focus on generating video descriptions based on the identification of (subject, verb, object) triplets with visual classifiers.
%The captions were generated through a language model which fitted predicted triplets to predefined sentence templates.
However, such the template-based approaches have limited ability to generalize to unseen data, and the generated sentences cannot satisfy the richness of natural language.
Inspired by the success of deep neural networks in neural machine translation (NMT) and image captioning~\cite{vinyals2015show,karpathy2015deep}.
Some researchers have moved to the use of recurrent neural networks (RNNs), which, given a vectored description of a visual content, could naturally deal with sequences of words~\cite{vinyals2015show,karpathy2015deep}.
%\subsubsection{video captioning with RNN network:}
%One of the first approaches of video captioning with recurrent neural networks,

%\subsubsection{video captioning with attribute detection}
The first work generalize RNNs to video captioning is~\cite{venugopalan2014translating}, in which they proposed an encoder-decoder based framework for video caption generation.
They used CNN to extract features from the single frame, and take an average pooling over them to get the entire video representation. They use a LSTM network as the sentence decoder.
However, their mean pooling operation ignored the sequential nature of videos.
After that, many works have tried to improve the video encoding process.
In \cite{donahue2015long}, they encoded the input video with a LSTM network and employed CRFs to to generate coherent video description.
Venugopalan et. al.~\cite{venugopalan2015sequence} encode the video with a stacked LSTM network, and another LSTM network to generate the video description.
Their framework was latter improved by incorporating attention mechanisms~\cite{yao2015describing} in the sentence decoder, or combining external knowledge with sentence decoders~\cite{rohrbach2015long}.

%\subsubsection{video captioning with attribute detection} 
To generate more accurate captions, attribute detections are involved in the model to detect the semantic attributes of a frame. Each element in an attribute vector represents the possibility of a semantic attribute appearing in the frames. Pan et. al. \cite{pan2017video} propose a video captioning model combined with semantic attribute detection. They propose a Transfer Unit to merge the temporal information with the image attributes and video attributes. To further improve this method, Gan et. al. \cite{gan2017semantic} propose an individual LSTM structure using the semantic information to guide the weight matrix in an LSTM. With the new structure, the semantic information is involved in language decoding process rather than merging with the hidden state to generate a fused vector. Although the methods perform well in video captioning, they can not get a good result by only training with a video captioning dataset because the video captioning datasets usually do not contain enough data to train a good attribute detection. The method all involve an additional image dataset to train the image attribute detection network.

Pasunuru also proposes a work et. al. \cite{pasunuru2017multi}  requiring the multi-dataset for training. They add a video prediction and entailment generation into the video captioning task to learning better representations of both video and language side. They involve the UFC-101 action videos dataset to train the video prediction model and the Stanford Natural Language Inference (SNLI) corpus to train the entitlement generation. 

%\subsubsection{video captioning with hierarchical structure}
Comparing with the simple encoder-decoder structure, the hierarchical structure introduces multiple layers into the model to learning different information in a different layer. Song et. al. \cite{song2017hierarchical} proposed a hierarchical language decoder to generate a sentence considering both low-level visual information and high-level language context information. They propose an adjusted component to merge the attended vector and hidden state of language decoder. In this way.the model involves more direct video information generate the words whose attributes appear in the video. On the other hand, the video encoder can also be enhanced with a hierarchical structure. Pan et. al. \cite{pan2016hierarchical}
propose a two-layer RNN video encoder to model the temporal information efficiently by control the length of the video information flow. Different from the stack RNN in sequence-to-sequence method , they introduce a hierarchical video encoder with a variant encoding interval. The low-level LSTM filter encodes the video feature in the chunks which contains the same amount of features. The high-level encoder encodes the final outputs of LSTM filter to generate an encoded vector containing the global understanding of the video. With the LSTM filter, the model can fully use whole frames in the video instead of select several keyframes from them and model the long-range dependency more efficiently.

Baraldi et. al. \cite{baraldi2016hierarchical} propose a boundary-aware method for video encoding model which can be view as the extension of Pan's work \cite{pan2016hierarchical}. They introduce a boundary detection into LSTM to decide hong long a chunk is automatically. The low-level LSTM encodes the features in a chunk to generate a set of hidden states. Then the high-level LSTM encodes the final hidden states of each chunk to generate a global undersatnding of the video.

Our approach involves a video prediction process to force the video encoding part to learn a better representation. Different from the approach proposed by Pasunuru et. al. \cite{pasunuru2017multi}, we also share the soft attention model with the video captioning process which proved better than the indiviual attention models for each process. Our approach involves the boundary detection to detect the video boundary. Additionally, we propose a individual RNN structure to detection the language boundary in parallel with a hierarchical language model. Different from the boundary-aware model, we input a global information of language generation to detect if there is a boundary instead of the information of current encoded feature applied in approach \cite{baraldi2016hierarchical}.



